Generalized Rindler Wedge and Holographic Observer Concordance

Defining gravitational subsystems has long been challenging due to the lack of the conventional notion of locality in gravity. In this work, we define gravitational subsystems from the observable spacetime subregions of a set of well-defined accelerating observers. We study the most general horizons of accelerating observers and find that in a general spacetime, only spacelike surfaces satisfying a global condition could become horizons of well-defined accelerating observers, which we name the Rindler-convexity condition. The entanglement entropy associated with a Rindler-convex region is proportional to the area of the enclosing surface. The subregions defined from this observer perspective is named the generalized Rindler wedge. This provides a physical origin for defining gravitational subsystems associated with one type of Type III von Neumann subalgebra. We propose the holographic interpretation of generalized Rindler wedges and provide evidence from the observer correspondence, the subregion subalgebra duality, and the equality of the entanglement entropy, respectively. We introduce time/space cutoffs in the bulk to substantiate this proposition, generalize it, and establish a holographic observer concordance framework, which asserts that the partitioning of degrees of freedom through observation is holographically concordant.

==> old_ref.tex <==
@article{Ju:2023dzo,
    author = "Ju, Xin-Xiang and Liu, Bo-Hao and Pan, Wen-Bin and Sun, Ya-Wen and Wang, Yuan-Tai",
    title = "{Squashed Entanglement from Generalized Rindler Wedge}",
    eprint = "2310.09799",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "10",
    year = "2023"
}

@article{Ju:2023,
  title={work in progress},
  author={Ju, Xin-Xiang and Pan, Wen-Bin and Wang, Yuan-Tai and Sun, Ya-Wen},
}

@article{galloway1989some,
  title={Some connections between global hyperbolicity and geodesic completeness},
  author={Galloway, Gregory J},
  journal={Journal of Geometry and Physics},
  volume={6},
  number={1},
  pages={127--141},
  year={1989},
  publisher={Elsevier}
}

@article{Headrick:2007km,
   author = "Headrick, Matthew and Takayanagi, Tadashi",
   title = "{A Holographic proof of the strong subadditivity of entanglement entropy}",
   eprint = "0704.3719",
   archivePrefix = "arXiv",
    primaryClass = "hep-th",
   reportNumber = "SU-ITP-07-08, KUNS-2069",
   doi = "10.1103/PhysRevD.76.106013",
   journal = "Phys. Rev. D",
   volume = "76",
    pages = "106013",
    year = "2007"
}

@book{Hawking:1973uf,
    author = "Hawking, S. W. and Ellis, G. F. R.",
    title = "{The Large Scale Structure of Space-Time}",
    doi = "10.1017/CBO9780511524646",
    isbn = "978-0-521-20016-5, 978-0-521-09906-6, 978-0-511-82630-6, 978-0-521-09906-6",
    publisher = "Cambridge University Press",
    series = "Cambridge Monographs on Mathematical Physics",
    month = "2",
    year = "2011"
}

@article{dong2016reconstruction,
  title={Reconstruction of bulk operators within the entanglement wedge in gauge-gravity duality},
  author={Dong, Xi and Harlow, Daniel and Wall, Aron C},
  journal={Physical review letters},
  volume={117},
  number={2},
  pages={021601},
  year={2016},
  publisher={APS}
}

@article{Bousso:2015mqa,
    author = "Bousso, Raphael and Engelhardt, Netta",
    title = "{New Area Law in General Relativity}",
    eprint = "1504.07627",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevLett.115.081301",
    journal = "Phys. Rev. Lett.",
    volume = "115",
    number = "8",
    pages = "081301",
    year = "2015"
}

@article{Balasubramanian:2018uus,
    author = "Balasubramanian, Vijay and Rabideau, Charles",
    title = "{The dual of non-extremal area: differential entropy in higher dimensions}",
    eprint = "1812.06985",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP09(2020)051",
    journal = "JHEP",
    volume = "09",
    pages = "051",
    year = "2020"
}

@article{Engelhardt:2018kzk,
    author = "Engelhardt, Netta and Fischetti, Sebastian",
    title = "{Losing the IR: a Holographic Framework for Area Theorems}",
    eprint = "1805.08891",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1088/1361-6382/aafa0b",
    journal = "Class. Quant. Grav.",
    volume = "36",
    number = "3",
    pages = "035008",
    year = "2019"
}

@article{Kelly:2013aja,
    author = "Kelly, William R. and Wall, Aron C.",
    title = "{Coarse-grained entropy and causal holographic information in AdS/CFT}",
    eprint = "1309.3610",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP03(2014)118",
    journal = "JHEP",
    volume = "03",
    pages = "118",
    year = "2014"
}

@article{Bousso:1999cb,
    author = "Bousso, Raphael",
    title = "{Holography in general space-times}",
    eprint = "hep-th/9906022",
    archivePrefix = "arXiv",
    reportNumber = "SU-ITP-99-24",
    doi = "10.1088/1126-6708/1999/06/028",
    journal = "JHEP",
    volume = "06",
    pages = "028",
    year = "1999"
}

@article{Engelhardt:2015dta,
    author = "Engelhardt, Netta and Fischetti, Sebastian",
    title = "{Covariant Constraints on Hole-ography}",
    eprint = "1507.00354",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1088/0264-9381/32/19/195021",
    journal = "Class. Quant. Grav.",
    volume = "32",
    number = "19",
    pages = "195021",
    year = "2015"
}

@article{Bousso:2015qqa,
    author = "Bousso, Raphael and Engelhardt, Netta",
    title = "{Proof of a New Area Law in General Relativity}",
    eprint = "1504.07660",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    doi = "10.1103/PhysRevD.92.044031",
    journal = "Phys. Rev. D",
    volume = "92",
    number = "4",
    pages = "044031",
    year = "2015"
}

@article{Bousso:2012mh,
    author = "Bousso, Raphael and Freivogel, Ben and Leichenauer, Stefan and Rosenhaus, Vladimir and Zukowski, Claire",
    title = "{Null Geodesics, Local CFT Operators and AdS/CFT for Subregions}",
    eprint = "1209.4641",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.88.064057",
    journal = "Phys. Rev. D",
    volume = "88",
    pages = "064057",
    year = "2013"
}

@article{Harlow:2018fse,
    author = "Harlow, Daniel",
    title = "{TASI Lectures on the Emergence of Bulk Physics in AdS/CFT}",
    eprint = "1802.01040",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.22323/1.305.0002",
    journal = "PoS",
    volume = "TASI2017",
    pages = "002",
    year = "2018"
}

@article{Hamilton:2006az,
    author = "Hamilton, Alex and Kabat, Daniel N. and Lifschytz, Gilad and Lowe, David A.",
    title = "{Holographic representation of local bulk operators}",
    eprint = "hep-th/0606141",
    archivePrefix = "arXiv",
    reportNumber = "CU-TP-1149",
    doi = "10.1103/PhysRevD.74.066009",
    journal = "Phys. Rev. D",
    volume = "74",
    pages = "066009",
    year = "2006"
}

@article{Emparan:2006ni,
    author = "Emparan, Roberto",
    title = "{Black hole entropy as entanglement entropy: A Holographic derivation}",
    eprint = "hep-th/0603081",
    archivePrefix = "arXiv",
    doi = "10.1088/1126-6708/2006/06/012",
    journal = "JHEP",
    volume = "06",
    pages = "012",
    year = "2006"
}

@article{Raviteja:2020fzt,
    author = "Raviteja, Konka and Gutti, Sashideep",
    title = "{Aspects of marginally trapped and antitrapped surfaces in a $D$-dimensional evolving dust model}",
    eprint = "2006.06468",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    doi = "10.1103/PhysRevD.102.024072",
    journal = "Phys. Rev. D",
    volume = "102",
    number = "2",
    pages = "024072",
    year = "2020"
}

@article{Kabat:2011rz,
    author = "Kabat, Daniel and Lifschytz, Gilad and Lowe, David A.",
    title = "{Constructing local bulk observables in interacting AdS/CFT}",
    eprint = "1102.2910",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.83.106009",
    journal = "Phys. Rev. D",
    volume = "83",
    pages = "106009",
    year = "2011"
}

@article{Jacobson:2003wv,
    author = "Jacobson, Ted and Parentani, Renaud",
    title = "{Horizon entropy}",
    eprint = "gr-qc/0302099",
    archivePrefix = "arXiv",
    doi = "10.1023/A:1023785123428",
    journal = "Found. Phys.",
    volume = "33",
    pages = "323--348",
    year = "2003"
}

@article{Eisert:2008ur,
    author = "Eisert, J. and Cramer, M. and Plenio, M. B.",
    title = "{Area laws for the entanglement entropy - a review}",
    eprint = "0808.3773",
    archivePrefix = "arXiv",
    primaryClass = "quant-ph",
    doi = "10.1103/RevModPhys.82.277",
    journal = "Rev. Mod. Phys.",
    volume = "82",
    pages = "277--306",
    year = "2010"
}

@article{Sugishita:2022ldv,
    author = "Sugishita, Sotaro and Terashima, Seiji",
    title = "{Rindler bulk reconstruction and subregion duality in AdS/CFT}",
    eprint = "2207.06455",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "YITP-22-70",
    doi = "10.1007/JHEP11(2022)041",
    journal = "JHEP",
    volume = "11",
    pages = "041",
    year = "2022"
}

@article{Hubeny:2012ry,
    author = "Hubeny, Veronika E.",
    title = "{Extremal surfaces as bulk probes in AdS/CFT}",
    eprint = "1203.1044",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "DCTP-12-15",
    doi = "10.1007/JHEP07(2012)093",
    journal = "JHEP",
    volume = "07",
    pages = "093",
    year = "2012"
}

@article{Bousso:2012sj,
    author = "Bousso, Raphael and Leichenauer, Stefan and Rosenhaus, Vladimir",
    title = "{Light-sheets and AdS/CFT}",
    eprint = "1203.6619",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.86.046009",
    journal = "Phys. Rev. D",
    volume = "86",
    pages = "046009",
    year = "2012"
}

@article{Laflamme:1987ec,
    author = "Laflamme, R.",
    title = "{Entropy of a Rindler Wedge}",
    doi = "10.1016/0370-2693(87)90799-4",
    journal = "Phys. Lett. B",
    volume = "196",
    pages = "449--450",
    year = "1987"
}

@article{Bousso:1999xy,
    author = "Bousso, Raphael",
    title = "{A Covariant entropy conjecture}",
    eprint = "hep-th/9905177",
    archivePrefix = "arXiv",
    reportNumber = "SU-ITP-99-23",
    doi = "10.1088/1126-6708/1999/07/004",
    journal = "JHEP",
    volume = "07",
    pages = "004",
    year = "1999"
}

@article{VanRaamsdonk:2010pw,
    author = "Van Raamsdonk, Mark",
    title = "{Building up spacetime with quantum entanglement}",
    eprint = "1005.3035",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1142/S0218271810018529",
    journal = "Gen. Rel. Grav.",
    volume = "42",
    pages = "2323--2329",
    year = "2010"
}

@article{Czech:2012be,
    author = "Czech, Bartlomiej and Karczmarek, Joanna L. and Nogueira, Fernando and Van Raamsdonk, Mark",
    title = "{Rindler Quantum Gravity}",
    eprint = "1206.1323",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1088/0264-9381/29/23/235025",
    journal = "Class. Quant. Grav.",
    volume = "29",
    pages = "235025",
    year = "2012"
}

@article{Fursaev:1995ef,
    author = "Fursaev, Dmitri V. and Solodukhin, Sergey N.",
    title = "{On the description of the Riemannian geometry in the presence of conical defects}",
    eprint = "hep-th/9501127",
    archivePrefix = "arXiv",
    reportNumber = "JINR-E2-95-28, JINR, E2-95-28",
    doi = "10.1103/PhysRevD.52.2133",
    journal = "Phys. Rev. D",
    volume = "52",
    pages = "2133--2143",
    year = "1995"
}

@article{Banados:1993qp,
    author = "Banados, Maximo and Teitelboim, Claudio and Zanelli, Jorge",
    title = "{Black hole entropy and the dimensional continuation of the Gauss-Bonnet theorem}",
    eprint = "gr-qc/9309026",
    archivePrefix = "arXiv",
    reportNumber = "IASSNS-HEP-93-53",
    doi = "10.1103/PhysRevLett.72.957",
    journal = "Phys. Rev. Lett.",
    volume = "72",
    pages = "957--960",
    year = "1994"
}

@article{Parikh:2012kg,
    author = "Parikh, Maulik and Samantray, Prasant",
    title = "{Rindler-AdS/CFT}",
    eprint = "1211.7370",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP10(2018)129",
    journal = "JHEP",
    volume = "10",
    pages = "129",
    year = "2018"
}

@article{Bousso:2015mna,
    author = "Bousso, Raphael and Fisher, Zachary and Leichenauer, Stefan and Wall, Aron C.",
    title = "{Quantum focusing conjecture}",
    eprint = "1506.02669",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.93.064044",
    journal = "Phys. Rev. D",
    volume = "93",
    number = "6",
    pages = "064044",
    year = "2016"
}

@article{Harlow:2014yka,
    author = "Harlow, Daniel",
    title = "{Jerusalem Lectures on Black Holes and Quantum Information}",
    eprint = "1409.1231",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/RevModPhys.88.015002",
    journal = "Rev. Mod. Phys.",
    volume = "88",
    pages = "015002",
    year = "2016"
}

@article{Headrick:2019eth,
    author = "Headrick, Matthew",
    title = "{Lectures on entanglement entropy in field theory and holography}",
    eprint = "1907.08126",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "BRX-TH-6653",
    month = "7",
    year = "2019"
}

@article{Almheiri:2020cfm,
    author = "Almheiri, Ahmed and Hartman, Thomas and Maldacena, Juan and Shaghoulian, Edgar and Tajdini, Amirhossein",
    title = "{The entropy of Hawking radiation}",
    eprint = "2006.06872",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/RevModPhys.93.035002",
    journal = "Rev. Mod. Phys.",
    volume = "93",
    number = "3",
    pages = "035002",
    year = "2021"
}

@article{Balasubramanian:2022lnw,
    author = "Balasubramanian, Vijay and Lawrence, Albion and Magan, Javier M. and Sasieta, Martin",
    title = "{Microscopic origin of the entropy of astrophysical black holes}",
    eprint = "2212.08623",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "12",
    year = "2022"
}

@misc{https://doi.org/10.48550/arxiv.1806.06373,
  doi = {10.48550/ARXIV.1806.06373},
  
  url = {https://arxiv.org/abs/1806.06373},
  
  author = {Vishnoi, Nisheeth K.},
  
  keywords = {Optimization and Control (math.OC), Data Structures and Algorithms (cs.DS), Machine Learning (cs.LG), Differential Geometry (math.DG), FOS: Mathematics, FOS: Mathematics, FOS: Computer and information sciences, FOS: Computer and information sciences},
  
  title = {Geodesic Convex Optimization: Differentiation on Manifolds, Geodesics, and Convexity},
  
  publisher = {arXiv},
  
  year = {2018},
  
  copyright = {arXiv.org perpetual, non-exclusive license}
}

@article{Page:1993df,
    author = "Page, Don N.",
    title = "{Average entropy of a subsystem}",
    eprint = "gr-qc/9305007",
    archivePrefix = "arXiv",
    reportNumber = "ALBERTA-THY-22-93",
    doi = "10.1103/PhysRevLett.71.1291",
    journal = "Phys. Rev. Lett.",
    volume = "71",
    pages = "1291--1294",
    year = "1993"
}

@book{Carroll:2004st,
    author = "Carroll, Sean M.",
    title = "{Spacetime and Geometry}",
    isbn = "978-0-8053-8732-2, 978-1-108-48839-6, 978-1-108-77555-7",
    publisher = "Cambridge University Press",
    month = "7",
    year = "2019"
}

@article{Ryu:2006bv,
    author = "Ryu, Shinsei and Takayanagi, Tadashi",
    title = "{Holographic derivation of entanglement entropy from AdS/CFT}",
    eprint = "hep-th/0603001",
    archivePrefix = "arXiv",
    reportNumber = "NSF-KITP-06-11",
    doi = "10.1103/PhysRevLett.96.181602",
    journal = "Phys. Rev. Lett.",
    volume = "96",
    pages = "181602",
    year = "2006"
}

@article{Ryu:2006ef,
    author = "Ryu, Shinsei and Takayanagi, Tadashi",
    title = "{Aspects of Holographic Entanglement Entropy}",
    eprint = "hep-th/0605073",
    archivePrefix = "arXiv",
    reportNumber = "NSF-KITP-06-31, KUNS-2021",
    doi = "10.1088/1126-6708/2006/08/045",
    journal = "JHEP",
    volume = "08",
    pages = "045",
    year = "2006"
}

%First proposal of time-dependent “covariant” HEE, historically named as HRT formula. 
@article{Hubeny:2007xt,
    author = "Hubeny, Veronika E. and Rangamani, Mukund and Takayanagi, Tadashi",
    title = "{A Covariant holographic entanglement entropy proposal}",
    eprint = "0705.0016",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "DCPT-07-13, KUNS-2069",
    doi = "10.1088/1126-6708/2007/07/062",
    journal = "JHEP",
    volume = "07",
    pages = "062",
    year = "2007"
}

% Momentum-space entanglement
@article{Balasubramanian:2011wt,
    author = "Balasubramanian, Vijay and McDermott, Michael B. and Van Raamsdonk, Mark",
    title = "{Momentum-space entanglement and renormalization in quantum field theory}",
    eprint = "1108.3568",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "UPR-1233-T",
    doi = "10.1103/PhysRevD.86.045014",
    journal = "Phys. Rev. D",
    volume = "86",
    pages = "045014",
    year = "2012"
}

@article{Maldacena:1997re,
    author = "Maldacena, Juan Martin",
    title = "{The Large N limit of superconformal field theories and supergravity}",
    eprint = "hep-th/9711200",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-97-A097, HUTP-98-A097",
    doi = "10.1023/A:1026654312961",
    journal = "Adv. Theor. Math. Phys.",
    volume = "2",
    pages = "231--252",
    year = "1998"
}

 % Rindler geodesics, EW and CW

@article{Saraswat:2020zzf,
    author = "Saraswat, Krishan and Afshordi, Niayesh",
    title = "{Extracting Hawking Radiation Near the Horizon of AdS Black Holes}",
    eprint = "2003.12676",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP02(2021)077",
    journal = "JHEP",
    volume = "02",
    pages = "077",
    year = "2021"
}

@article{Espindola:2018ozt,
    author = "Esp\'\i{}ndola, Ricardo and Guijosa, Alberto and Pedraza, Juan F.",
    title = "{Entanglement Wedge Reconstruction and Entanglement of Purification}",
    eprint = "1804.05855",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1140/epjc/s10052-018-6140-2",
    journal = "Eur. Phys. J. C",
    volume = "78",
    number = "8",
    pages = "646",
    year = "2018"
}



@article{Strominger:1996sh,
    author = "Strominger, Andrew and Vafa, Cumrun",
    title = "{Microscopic origin of the Bekenstein-Hawking entropy}",
    eprint = "hep-th/9601029",
    archivePrefix = "arXiv",
    reportNumber = "HUTP-96-A002, RU-96-01",
    doi = "10.1016/0370-2693(96)00345-0",
    journal = "Phys. Lett. B",
    volume = "379",
    pages = "99--104",
    year = "1996"
}

@article{Bekenstein:1973ur,
    author = "Bekenstein, Jacob D.",
    title = "{Black holes and entropy}",
    doi = "10.1103/PhysRevD.7.2333",
    journal = "Phys. Rev. D",
    volume = "7",
    pages = "2333--2346",
    year = "1973"
}

@article{Bekenstein:1974ax,
    author = "Bekenstein, Jacob D.",
    title = "{Generalized second law of thermodynamics in black hole physics}",
    doi = "10.1103/PhysRevD.9.3292",
    journal = "Phys. Rev. D",
    volume = "9",
    pages = "3292--3300",
    year = "1974"
}

@article{Hawking:1975vcx,
    author = "Hawking, S. W.",
    editor = "Gibbons, G. W. and Hawking, S. W.",
    title = "{Particle Creation by Black Holes}",
    doi = "10.1007/BF02345020",
    journal = "Commun. Math. Phys.",
    volume = "43",
    pages = "199--220",
    year = "1975",
    note = "[Erratum: Commun.Math.Phys. 46, 206 (1976)]"
}

@article{Bardeen:1973gs,
    author = "Bardeen, James M. and Carter, B. and Hawking, S. W.",
    title = "{The Four laws of black hole mechanics}",
    doi = "10.1007/BF01645742",
    journal = "Commun. Math. Phys.",
    volume = "31",
    pages = "161--170",
    year = "1973"
}

@article{tHooft:1993dmi,
    author = "'t Hooft, Gerard",
    title = "{Dimensional reduction in quantum gravity}",
    eprint = "gr-qc/9310026",
    archivePrefix = "arXiv",
    reportNumber = "THU-93-26",
    journal = "Conf. Proc. C",
    volume = "930308",
    pages = "284--296",
    year = "1993"
}

@article{Susskind:1994vu,
    author = "Susskind, Leonard",
    title = "{The World as a hologram}",
    eprint = "hep-th/9409089",
    archivePrefix = "arXiv",
    reportNumber = "SU-ITP-94-33",
    doi = "10.1063/1.531249",
    journal = "J. Math. Phys.",
    volume = "36",
    pages = "6377--6396",
    year = "1995"
}

@article{Rindler:1966zz,
    author = "Rindler, W.",
    title = "{Kruskal Space and the Uniformly Accelerated Frame}",
    doi = "10.1119/1.1972547",
    journal = "Am. J. Phys.",
    volume = "34",
    pages = "1174",
    year = "1966"
}

@article{Czech:2012bh,
    author = "Czech, Bartlomiej and Karczmarek, Joanna L. and Nogueira, Fernando and Van Raamsdonk, Mark",
    title = "{The Gravity Dual of a Density Matrix}",
    eprint = "1204.1330",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1088/0264-9381/29/15/155009",
    journal = "Class. Quant. Grav.",
    volume = "29",
    pages = "155009",
    year = "2012"
}

@article{Wall:2012uf,
    author = "Wall, Aron C.",
    title = "{Maximin Surfaces, and the Strong Subadditivity of the Covariant Holographic Entanglement Entropy}",
    eprint = "1211.3494",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1088/0264-9381/31/22/225007",
    journal = "Class. Quant. Grav.",
    volume = "31",
    number = "22",
    pages = "225007",
    year = "2014"
}



%%%%%%%%%%%%%%% Not cited %%%%%%%%%%%%%%%%%


@article{Faulkner:2013ana,
    author = "Faulkner, Thomas and Lewkowycz, Aitor and Maldacena, Juan",
    title = "{Quantum corrections to holographic entanglement entropy}",
    eprint = "1307.2892",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP11(2013)074",
    journal = "JHEP",
    volume = "11",
    pages = "074",
    year = "2013"
}

@article{Engelhardt:2014gca,
    author = "Engelhardt, Netta and Wall, Aron C.",
    title = "{Quantum Extremal Surfaces: Holographic Entanglement Entropy beyond the Classical Regime}",
    eprint = "1408.3203",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP01(2015)073",
    journal = "JHEP",
    volume = "01",
    pages = "073",
    year = "2015"
}

@article{Akers:2019lzs,
    author = "Akers, Chris and Engelhardt, Netta and Penington, Geoff and Usatyuk, Mykhaylo",
    title = "{Quantum Maximin Surfaces}",
    eprint = "1912.02799",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP08(2020)140",
    journal = "JHEP",
    volume = "08",
    pages = "140",
    year = "2020"
}


@article{Gibbons:1976ue,
    author = "Gibbons, G. W. and Hawking, S. W.",
    title = "{Action Integrals and Partition Functions in Quantum Gravity}",
    reportNumber = "PRINT-76-0995 (CAMBRIDGE)",
    doi = "10.1103/PhysRevD.15.2752",
    journal = "Phys. Rev. D",
    volume = "15",
    pages = "2752--2756",
    year = "1977"
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



@article{Leutheusser:2022bgi,
    author = "Leutheusser, Samuel and Liu, Hong",
    title = "{Subalgebra-subregion duality: emergence of space and time in holography}",
    eprint = "2212.13266",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "12",
    year = "2022"
}

@article{Balasubramanian:2013rqa,
  author        = {Balasubramanian, Vijay and Czech, Bartlomiej and Chowdhury, Borun D. and de Boer, Jan},
  title         = {{The entropy of a hole in spacetime}},
  eprint        = {1305.0856},
  archiveprefix = {arXiv},
  primaryclass  = {hep-th},
  doi           = {10.1007/JHEP10(2013)220},
  journal       = {JHEP},
  volume        = {10},
  pages         = {220},
  year          = {2013}
}

@article{Balasubramanian:2013lsa,
    author = "Balasubramanian, Vijay and Chowdhury, Borun D. and Czech, Bartlomiej and de Boer, Jan and Heller, Michal P.",
    title = "{Bulk curves from boundary data in holography}",
    eprint = "1310.4204",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1103/PhysRevD.89.086004",
    journal = "Phys. Rev. D",
    volume = "89",
    number = "8",
    pages = "086004",
    year = "2014"
}

@article{DeClerck:2019mkx,
    author = "De Clerck, Marine and Rabideau, Charles and Tanger, Niklas",
    title = "{Caustics bounding entanglement wedges}",
    eprint = "1912.09515",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP06(2020)166",
    journal = "JHEP",
    volume = "06",
    pages = "166",
    year = "2020"
}

@article{Lewkowycz:2013nqa,
    author = "Lewkowycz, Aitor and Maldacena, Juan",
    title = "{Generalized gravitational entropy}",
    eprint = "1304.4926",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP08(2013)090",
    journal = "JHEP",
    volume = "08",
    pages = "090",
    year = "2013"
}
@article{Headrick:2014eia,
    author = "Headrick, Matthew and Myers, Robert C. and Wien, Jason",
    title = "{Holographic Holes and Differential Entropy}",
    eprint = "1408.4770",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "BRX-TH-6283",
    doi = "10.1007/JHEP10(2014)149",
    journal = "JHEP",
    volume = "10",
    pages = "149",
    year = "2014"
}
@article{Prihadi:2022lsw,
    author = "Prihadi, Hadyan Luthfan and Zen, Freddy Permana and Ariwahjoedi, Seramika and Dwiputra, Donny",
    title = "{Replica Trick Calculation for Entanglement Entropy of Static Black Hole Spacetimes}",
    eprint = "2208.01829",
    archivePrefix = "arXiv",
    primaryClass = "gr-qc",
    month = "8",
    year = "2022"
}
@article{Bousso:2022hlz,
    author = "Bousso, Raphael and Penington, Geoff",
    title = "{Entanglement Wedges for Gravitating Regions}",
    eprint = "2208.04993",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    month = "8",
    year = "2022"
}

@article{Headrick:2014cta,
    author = "Headrick, Matthew and Hubeny, Veronika E. and Lawrence, Albion and Rangamani, Mukund",
    title = "{Causality \& holographic entanglement entropy}",
    eprint = "1408.6300",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "DCPT-14-33, BRX-TH-6284",
    doi = "10.1007/JHEP12(2014)162",
    journal = "JHEP",
    volume = "12",
    pages = "162",
    year = "2014"
}

@article{Brown:2019rox,
    author = "Brown, Adam R. and Gharibyan, Hrant and Penington, Geoff and Susskind, Leonard",
    title = "{The Python\textquoteright{}s Lunch: geometric obstructions to decoding Hawking radiation}",
    eprint = "1912.00228",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP08(2020)121",
    journal = "JHEP",
    volume = "08",
    pages = "121",
    year = "2020"
}

@article{Hubeny:2012wa,
    author = "Hubeny, Veronika E. and Rangamani, Mukund",
    title = "{Causal Holographic Information}",
    eprint = "1204.1698",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "DCPT-12-21",
    doi = "10.1007/JHEP06(2012)114",
    journal = "JHEP",
    volume = "06",
    pages = "114",
    year = "2012"
}


@article{Penington:2019npb,
    author = "Penington, Geoffrey",
    title = "{Entanglement Wedge Reconstruction and the Information Paradox}",
    eprint = "1905.08255",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    doi = "10.1007/JHEP09(2020)002",
    journal = "JHEP",
    volume = "09",
    pages = "002",
    year = "2020"
}

@article{Leutheusser:2021qhd,
    author = "Leutheusser, Samuel and Liu, Hong",
    title = "{Causal connectability between quantum systems and the black hole interior in holographic duality}",
    eprint = "2110.05497",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "MIT-CTP/5335",
    month = "10",
    year = "2021"
}

@article{Lieb:1973cp,
    author = "Lieb, E. H. and Ruskai, M. B.",
    title = "{Proof of the strong subadditivity of quantum-mechanical entropy}",
    doi = "10.1063/1.1666274",
    journal = "J. Math. Phys.",
    volume = "14",
    pages = "1938--1941",
    year = "1973"
}

@book{Wald:1984rg,
    author = "Wald, Robert M.",
    title = "{General Relativity}",
    doi = "10.7208/chicago/9780226870373.001.0001",
    publisher = "Chicago Univ. Pr.",
    address = "Chicago, USA",
    year = "1984"
}

@article{Akal:2021csd,
    author = "Akal, Ibra",
    title = "{Information storage and near horizon quantum correlations}",
    eprint = "2109.01639",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "YITP-21-90",
    month = "9",
    year = "2021"
}

@article{Akal:2021foz,
    author = "Akal, Ibrahim and Kusuki, Yuya and Shiba, Noburo and Takayanagi, Tadashi and Wei, Zixia",
    title = "{Holographic moving mirrors}",
    eprint = "2106.11179",
    archivePrefix = "arXiv",
    primaryClass = "hep-th",
    reportNumber = "YITP-21-53, IPMU21-0035, RIKEN-iTHEMS-Report-21",
    doi = "10.1088/1361-6382/ac2c1b",
    journal = "Class. Quant. Grav.",
    volume = "38",
    number = "22",
    pages = "224001",
    year = "2021"
}


